The Influence Operation Ontology (IOO)

Ontologies provide a systematic framework for organizing and leveraging knowledge, enabling smarter and more effective decision-making. In order to advance in the capitalization and augmentation of intelligence related to nowadays cyberoperations, the proposed Influence Operation Ontology (IOO) establishes the main entities and relationships to model offensive tactics and techniques by threat actors against the public audience through the information environment. It aims to stimulate research and development in the field, leading to innovative applications against influence operations, particularly in the fields of intelligence, security, and defense.

==> aux.tex <==
Disinformation campaigns have become a less of a rarity in the last years.
While propaganda, deception and influence operations are not new in the geopolitical landscape \cite{mildec},
the scale of social media in all its forms are.
Platforms such as X, Facebook or Instagram has worsned the effect of these practices, as now, 
news and opinions by anyone can go viral at the speed of a click.

As a reference, the Ukranian war has served as the perfect scenario
for these disinformation campaings to prolifierate,
where social media platforms have played an essential role for spreading
disinformation about war events by influencing users all around the world
and shaping the public opinions of countries, 
resulting in expectations "of the people for the rulers to do something".

Political powers are now more aware than never about the nature of disinformation
in the cyberspace \cite{} \cite{}. %eaas
The increase in the scale of disinformation incidents has 
developed a need for structured ways of modeling this theats
that could result in a more informed analisys and understanding about them.

As the Internet and social networks are now the main drivers of disinformation campaigns,
we can consider them as a cybersecurity and cyberdefense concern.
This means that cybersecurity incidents, tools and processes can be thought as possible 
alternatives to combat disinformation, specially when dealing with large scale campaigns 
with other technical malicious activities such as botnets, malicious ads, etc.

To address this, some frameworks that take advantages of already known cybersecurity practices and tools
have been developed with a good welcome by practitioners,
serving them as a useful tool for combating disinformation by
having an structured language and workflow.
Aditionally, it exists some initiatives that tries to map the tactics 
proposed by these identified common tactics to 
a CTI languages, so disinformation incidents can be easily ingested and undertood
by CTI platforms, which have been prove useful in managing cybersecurity threats \cite{}.

However, still exist a lack of platforms that take advantage of 
the CTI nature of this frameworks to create a repository of disinformation incidents
that is able of programatically ingesting/extracting structured objects from CTI platforms.
This way, an automatic system capable handling of large amount of disinformation incidents can be created to manage the reports being produced on a monthly basis.
Specifically, the main objectives of this platform are:
\begin{itemize}
    \item Study of the main proposals for disinformation threat modelling?.
    \item Demonstrate the implementation of structured languages for disinformation modelling.
    \item Develop a centralized platform capable of visualizing and exchanging disinformation incidents to CTI solutions and accepting incidents uploaded by non-technical users like reporters.
\end{itemize}



In order to identify the correct elements and functionalities to design the platform, several steps were taken:

Firstly, a framework to model disinformation incidents had to be chosen, 
as these events are often very complex and a tool is needed to syntethize some of its details in other simpler computable elements.
Ideally, This framework would  be oriented to cybersecurity, being able to characterize disinformation
elements into fixed concepts like TTPs or Cyber Kill Chain steps.
For this, the results of \cite{disinfomodel} were acknowledged,
checking all the pros and cons of all the analyzed frameworks.
Among all the analyzed frameworks, the one that fitted our use case the best was the DISARM Framework
as it provides a cybersecurity oriented way of analyzing a disinformation incident
due to its MITRE-like matrix with TTPs and Cyber Kill Chain-like phases.
Most importantly, the DISARM framework already provides examples of how its TTPs can
be treated as STIX2 objects, having also an official connector that inserts these objects
to the OpenCTI platform for manual correlation inside it, 
which can be considered a good first aproach to look on for developing DISINFOX.

Secondly, an specific data model was defined to represent the disinformation incidents.
Although DISARM already transform its TTPs and matrix with its official DISARM STIX2 Generator,
this do not offer guidance on how an incident could be represented with DISARM in STIX2.
Therefore, an specific binding was created between the different elements that an incident could have
and their corresponding translation to STIX2 objects.

Thirdly, a design phase was performed in which the main elements of the platform were 
selected taking into account the main objectives and requirements of this work.
Here, the architecture, database mode, language and scope were defined to have a wireframe of
what it was needed to be built.

Lastly, the development phase was performed. 
In this case, an iterative aproach was followed by adding incremental elements, features and changes
to the codebase.


For the solution to be CTI-compatible, STIX2 objects were used to provide interoperability between connectors using this standard.

However, although there are intuitive and standardized ways the different evidence of cybersecurity incidents to STIX2 objects,
there are no standard that guides the transformation of disinformation incidents.

Therefore, efforts were made to abstract the nature of disinformation incidents 
to fit them in the already available STIX2 objects, 
providing an equivalency between a disinformation incident and a cybersecurity incident.

In Table \ref{tab:mapping} we can see the equivalency presented to store the obtained
disinformation incidents and its pieces of evidence into STIX2 objects:
\begin{itemize}
    \item The Incident is the core element of a disinformation incident,
    with important properties suchas:  name, description, etc.
    It will be link all the other objects related with the incident.
    It is mapped to  Intrusion Set as this is a group of actions and resources
    leveraged by a certain entity, which is similar to what is known as a disinformation incident.
    \item The Actor is the organization or individual who is believed to be the author
    of the Incident.
    It is mapped to ThreatActor as 
\end{itemize}


\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{ l  l  X }
    %\begin{tabularx}{\textwidth}{bss}
        \hline
        \textbf{Disinformation evidences}     & \textbf{STIX2 equivalency}  & \textbf{Reason}     \\ \hline
        Incident         & Intrusion Set  &            \\ \hline
        Actor         & Threat Actor     &         \\ \hline
        Affected Country & Country & \\ \hline
        Detected Techniques  & Attack Pattern & \\ \hline

    \end{tabularx}
    \caption{Mapping between disinformation evidences and STIX2 objects}
    \label{tab:mapping}
\end{table}

==> itemize_aux.tex <==
%%%% Incident %%%%%%


\begin{itemize}
 \item Name: a name to identify the incident. 
 \item Description: a description of the incident providing more context and details, usually including its purpose and what happened.  
 \item First seen: the first time that the incident was seen. 
 \item Last seen: the last time that the incident was seen.
 \item Objective: this is the primary goal, objective, desired outcome, or intended effect.
\end{itemize}




%%% Attack Pattern %%%% 


\begin{itemize}
 \item Name: a name to identify the attack pattern. 
 \item Description: a description of the attack pattern providing more context and details, potentially including its purpose and key characteristics.
 \item Alias: alternative names used to identify the attack pattern.
 \item External reference: the technique of the attack pattern from de DISARM Framework~\cite{disarm_framework}.  
 \item Kill chain phase:  the tactic of the attack pattern from de DISARM Framework~\cite{disarm_framework} or the phase of Disarm Kill Chain~\cite{filigran}.
\end{itemize}




%%% Campaign %%%%



\begin{itemize}
 %\item Id: 
 \item Name: a name to identify the campaign. 
 \item Description: a description of the Campaign providing more context and details, usually that description includes its purpose and its key characteristics.  
 \item Aliases: a list of other names that identify (or are believed to identify) this threat actor.
 \item First seen: the first time that the campaign was seen. 
 \item Last seen: the last time that the campaign was seen.
 \item Objective: this is the primary goal, objective, desired outcome, or intended effect. That is, what the threat actor or intrusion set wants to achieve with this campaign. 
\end{itemize}



%%% Threat Actor %%%%%

\begin{itemize}
 \item Name: a name to identify the threat actor or threat actor group. 
 \item Description: a detailed description of the threat actor that usually includes its purpose and its key characteristics. % STIX Version 2.1 
 \item Threat actor type: the type(s) of this threat actor. % STIX Version 2.1
 \item Aliases: a list of other names that identify (or are believed to identify) this threat actor.
 \item First seen: the first time the threat actor was seen. 
 \item Last seen: the last time the threat actor was seen.
 \item Roles:  the type(s) of this threat actor. For example, activists, proxies, crime syndicates, nation-states, and so on. Not mutually exclusive.
 \item Goals: describe what is the threat actor trying to do. 
 \item Sophistication: the level of skill, specialized knowledge, training, or expertise required for a threat actor to execute an attack.
 \item Resource level: The organizational tier at which the threat actor typically operates, determining the resources available to support their attacks.
 \item Primary motivations: The core reasons, intentions, or objectives driving the threat actor’s actions, defining what they aim to achieve.
 \item Secondary motivations: additional reasons, motivations, or purposes influencing the threat actor. These may complement the primary motivation but do not necessarily amplify or replace it, instead providing further context. 
 \item Personale motivations: the individual reasons or desires that drive a threat actor’s actions, independent of their organization’s goals. While personal motivations can align with organizational objectives, as seen with activists, they often serve personal interests rather than collective agendas.
\end{itemize}




%%%%%%%%%%%%%% Target Domain %%%%%%%%%%%%%%%%%%%%%%%%%

%%% Entity %%%%%

\begin{comment}
\begin{itemize}
 %\item Id: 
 \item Name: a name to identify the entity. 
 \item Description: a description that provides more details and context about the Target, potentially including its purpose and its key characteristics. 
 %\item Role: Begins to Cyber persona I think. 
 %\item Identity class: indicates the type of the Target, e.g., individual, organization, and so on. 
 \item Sector: industry sectors where the entity belongs to. 
\end{itemize}
\end{comment}


%%% Location %%%%%

\begin{comment}
\begin{itemize}
 \item Name: a name used to identify the location. 
 \item Description: a textual description of the location.
 \item Latitude: the location's latitude in decimal degrees, where positive values indicate positions north of the equator and negative values represent positions south of the equator. 
 \item Longitude: the location's longitude in decimal degrees, where positive values indicate longitudes east of the prime meridian and negative values indicate longitudes west of the prime meridian.
 \item Precision: defines the precision of the coordinates specified by the latitude and longitude properties. 
 \item Region: the region that this location describes. 
 \item Country: the country that this location describes.
 \item Administrative area: The state, province, or other sub-national administrative area that this location describes (ISO 3166-2 Code).
 \item City: the city that this location describes.
 \item Street address:  the street address that this location describes.
 \item Postal code: the postal code for this location.
\end{itemize}
\end{comment}



%%%%%%%%%%%%%% Channel Domain %%%%%%%%%%%%%%%%%%%%%%%%


%%% Channel %%%%%

\begin{comment}
\begin{itemize}
 \item Name: a name to identify the Channel.  
 \item Description: a detailed explanation of the Channel, including its function, relevance, and role in message dissemination.  
 \item Type: the kind of platform or medium used.
 \item Affiliation: any known connection to organizations, networks, or influence operations.  
 \item Reach: the estimated audience size and engagement level of the Channel.  
 \item Purpose: the primary goal of the Channel.
 \item Sponsored: whether the Channel is financially supported or promoted by an external entity, such as a government or private organization.
 \item Channel Type: the classification of the channel based on its affiliation and control structure (e.g official Communication Channel, State-linked channels, State-controlled Channels).
\end{itemize}
\end{comment}


%%% Message %%%%%

\begin{comment}
\begin{itemize}
 \item Name: a name to identify the Message.  
 \item Description: a detailed message explanation, including its purpose, main topic, and relevant contextual information.  
 \item Media content: the multimedia elements associated with the Message, such as text, images, videos, or audio.  
 \item URL: the web address where the Message is hosted or published.  
 \item Format: the type of Message, e.g., tweet, article, video, news report, or social media post.    
\end{itemize}
\end{comment}


%%% User-account %%%%%
\begin{comment}
\begin{itemize}
    \item Display name: the public name of the user account, which may differ from the actual name.
    \item Name: the real or chosen name associated with the account.
    \item Age: the age of the account owner.
    \item Icon: the profile image or avatar representing the account.
    \item Description: a brief bio or tagline summarizing the user’s purpose, interests, or affiliations.
    \item External links: URLs linking to other profiles, websites, or resources related to the account.
    \item Region: the geographical location associated with the account.
    \item Account created: the date when the account was registered on the platform.
    \item Platform: the specific internet service or social media network where the account operates.
    \item Privacy settings: the level of visibility (public, private, restricted) set by the user.
    \item Followers: the number of users who subscribe to or follow the account’s updates.
    \item Following: The number of other accounts this user follows.
    \item Rating: a metric that reflects the account's reputation, trust, or engagement level.
    \item Privileged: indicates whether the account has special privileges (e.g., verified status, admin rights).
    \item Disabled: specifies whether the account is active, suspended, or permanently banned.
    \item Bot: a number that indicates the automatic actions' level.
\end{itemize}
\end{comment}





%%%%%%%%%%%%%% Social Domain %%%%%%%%%%%%%%%%%%%%%%%%


%%%%%% Cyber persona %%%%%%  
\begin{comment}
    

\begin{itemize}
    \item Name: the real name of the cyber persona.
    \item Alias: alternative names, usernames, or pseudonyms the cyber persona uses in digital environments.  
    \item Age: the age of the cyber persona, whether real or self-reported.  
    \item Description: A brief bio summarizing the cyber persona’s physical characteristics, interests, affiliations, or online presence. 
    \item Gender: gender with which the cyber persona identifies itself.
    \item Language: the primary language(s) used by the cyber persona.
    \item Religion: the religious beliefs, or ideologies associated with the cyber persona.  
    \item Ethic: 
    \item Occupation: the profession, role, or function of the cyber persona.
    \item Interest: topics, activities, or fields of engagement of the cyber persona.
    \item Opinions: expressed viewpoints, perspectives, or ideological positions that the cyber persona actively shares or supports online.
    \item Values: core beliefs and guiding principles that influence the cyber persona’s behavior and decision-making.  
    \item Behavioral: recognized behavioral patterns, such as communication style, engagement frequency, and interaction strategies and tendencies.
    \item Affiliation: any known connection to organizations, networks, or influence operations.
\end{itemize}
\end{comment}



%%%%%% Community %%%%%%  

\begin{comment}
\begin{itemize}
 %\item Id: 
 \item Name: a name to identify the Community.  
 \item Description: a brief overview of the community, its purpose, and its main characteristics.  
 \item Type: the nature of the group, e.g., organization, corporate, social, ideological, or online.  
 \item Goal: the primary objective of the community, whether social, political, economic, or cultural.  
 \item Structure: how the community is organized.  
 \item Resources: the assets the community relies on, such as members, funding, information, or technology.  
 \item Topic: the central themes or issues that unite the community.  
 \item Values: the core principles or beliefs that guide the community's actions and cohesion.  
 \item Feature: defining characteristics that distinguish this community from others, such as exclusivity, openness, or interaction dynamics.  
\item Affiliation: any known connection to organizations, networks, or influence operations.
\end{itemize}
\end{comment}

%%%%%% Narrative %%%%%%  
\begin{comment}
\begin{itemize}
 \item Name: a name to identify the Narrative.  
 \item Description: a summary of the narrative's core content, context, and variations.  
 \item Goal: the main purpose of the narrative, what this narrative is trying to produce or obtain. 
 \item Topic: the central theme (politics, economy, health, security, etc.).  
 \item Actor:  the narrative stakeholders.
 \item Targeted Public: the intended audience based on demographics, psychographics, and online communities.  
 %\item Frame: how the narrative is structured and interpreted.   
 \item Emotion: the main emotions triggered by the narrative.  
 \item Affiliation: any known connection to organizations, networks, or influence operations.
\end{itemize}
\end{comment}
